Oh-RAM! One and a Half Round Atomic Memory

Emulating atomic read/write shared objects in a message-passing system is a fundamental problem in distributed computing. Considering that network communication is the most expensive resource, efficiency is measured first of all in terms of the communication needed to implement read and write operations. It is well known that 2 communication round-trip phases involving in total 4 message exchanges are sufficient to implemented atomic operations. It is also known that under certain constraints on the number of readers with respect to the numbers of replica servers and failures it is possible to implement single-writer atomic objects such that each operation involves one round-trip phase. We present algorithms that allow operations to complete in 3 communication exchanges without imposing any constraints on the number of readers and writers. Specifically, we present an atomic memory implementation for the SWMR setting, where reads complete in 3 communication exchanges and writes complete in 2 exchanges. We pose the question of whether it is possible to implement MWMR memory where operations complete in at most 3 communication exchanges. We answer this question in the negative by showing that an atomic memory implementation is impossible if both read and write operations take 3 communication exchanges, even when assuming two writers, two readers, and a single replica server failure. Motivated by this impossibility result, we provide a MWMR atomic memory implementation where reads involve 3 and writes 4 communication exchanges. In light of our impossibility result these algorithms are optimal in terms of the number of communication exchanges. We rigorously reason about the correctness of the algorithms.

==> Complexity_summary.tex <==
\section{Algorithms Complexity}
\label{sec:app_complexity}
%\input{app_complexity.tex}

We now assess the performance of our algorithms in terms of (i) latency of read and write operations
as measured by the number of communication exchanges, and (ii) the communication (message) complexity of read and write operations. 

\remove{The main two factors that affect the latency of each operation is (a) \emph{computation time} and (b) \emph{communication exchanges}. 

\paragraph{Computation Complexity.} This factor is measured by counting the steps that the algorithm takes each time it invokes an  operation. 
%
For algorithms \osam{} and \omam{} during any operation, process $\pr$ can receive up to $|\srvSet|$ messages. Since up to $|\srvSet|$ comparison steps can take place in each operation, the resulting computation complexity for each operation is $|\srvSet|$. 
 %
For algorithms \osamex{} and \omamex{}, during a read operation, the invoker process $\pr$ can receive up to $2|\srvSet|$ messages and perform $2|\srvSet|$ comparison steps. Thus the resulting computation complexity for a read operation is $2|\srvSet|$. Since write and server protocols are identical to the ones used in \osam{} and \omam{}, then as we analysed above any other operation has computation complexity of $|\srvSet|$.


\paragraph{Communication Complexity.} Latency  is measured in terms of communication exchanges. 
%(Definition \ref{def:metric}).  
Below we analyse the communication complexity for each read/write operation for all the algorithms. 
}%REMOVE

\ppp{Operation Latency.} ~


SWMR write operation latency:
%\paragraph{} \emph{SWMR write operation communication complexity.} 
According to algorithms \osam{} and \osamex{}, writer $w$ sends \emph{writeRequest} messages 
to all servers 
%$\srvr \in \srvSet$ 
and waits for \emph{writeAck} messages from a majority of servers. 
Once the \emph{writeAck} messages are received, no further communication is required and the write operation
terminates. Therefore, any write operation  consists of \emph{2} communication exchanges. 


MWMR write operation latency:
%\paragraph{} \emph{MWMR write operation communication complexity.} 
According to algorithms \omam{} and \omamex{}, writer $w$ sends \emph{discover} messages 
to all servers 
%$\srvr \in \srvSet$ 
and waits for \emph{discoverAck} messages from a majority of servers. 
Once the \emph{discoverAck} messages are received, then writer $w$ broadcasts 
a  \emph{writeRequest} message 
to all servers. 
It then waits for \emph{writeAck} messages from a majority of servers. 
No further communication is required and the write operation terminates. 
Thus any write operation  consists of \emph{4} communication exchanges.

SWMR and MWMR read operation latency in algorithms \osam{} and \omam{}:
%\paragraph{} \emph{Read operation (SWMR or MWMR) communication complexity.} 
A reader  sends \emph{readRequest} message to all servers
% $\srvr \in \srvSet$, forming 
in the first communication exchange. 
Once a server receives a \emph{readRequest} message, 
it broadcasts a \emph{readRelay} message to all servers
in the second communication exchange. 
Any active servers now await \emph{readRelay} messages from a majority of servers,
then the servers send a \emph{readAck} message to the reader
in the third communication exchange. 
We note that servers do not reply  to any incoming \emph{readRelay} messages. Therefore, read 
operations consists of \emph{3} communication exchanges.
% in both the SWMR and MWMR settings. 

SWMR and MWMR read operation latency in algorithms \osamex{} and \omamex{}:
%\paragraph{} \emph{Extended Read operation (SWMR or MWMR) communication complexity.} 
As before,
a reader  sends \emph{readRequest} message to all servers
in the first communication exchange.
Once the servers  receive the \emph{readRequest}
message they broadcast a \emph{readRelay} message to 
%(i) 
all  servers  \emph{and}
% (ii) 
the reader
in the second exchange.
The reader can terminate at the end of the second exchange
if it receives  \emph{readRelay} messages containing the same timestamp (\osamex{})
or tag (\omamex{}) values.
If this is not the case, the operation goes into the third exchange as in
algorithms  \osam{} and \omam{}.
Thus read operations terminate after either \emph{2} or \emph{3} communication exchanges.
%in both the SWMR and MWMR settings. 
\newline
\newline

\ppp{Communication (Message) Complexity.}

%\paragraph{Message Complexity.} 
We measure operation message complexity as the worst case number of exchanged messages 
in each read and write operation. 
The worst case number of messages corresponds to failure-free executions where all
participants send all messages according to the protocols. 

SWMR write operation message complexity:
Write operations in algorithms \osam{} and \osamex{}  take \emph{2} communication exchanges.
In the first exchange the writer sends a \emph{writeRequest} message to all servers in $\srvSet$.
The second exchange occurs when all servers in $\srvSet$ send a \emph{writeAck} message 
to the writer. 
Thus at most $2|\srvSet|$ messages are exchanged in any write operation.


{MWMR write operation message complexity:} 
Write operations in algorithms \omam{} and \omamex{} 
take \emph{4} communication exchanges. 
The first and the third exchange occur when a writer sends \emph{discover} and \emph{writeRequest} messages respectively to all servers in $\srvSet$. 
The second and fourth exchanges occur when servers in $\srvSet$ send \emph{discoverAck} and \emph{writeAck} messages respectively back to the writer. 
Thus $4|\srvSet|$ messages are exchanged in any write operation. 
%of Algorithm \ref{alg:trifastmwmr}. 

SWMR and MWMR read operation message complexity in algorithms \osam{} and \omam{}:
%\paragraph{} \emph{Read operation message complexity (SWMR and MWMR).} 
Read operations take  \emph{3} communication exchanges. 
The first exchange occurs when a reader  sends a \emph{readRequest} message to all servers in $\srvSet$. 
The second exchange occurs when  servers  in $\srvSet$ send \emph{readRelay} messages 
to all servers in $\srvSet$. 
The final exchange occurs when servers in $\srvSet$ send a \emph{readAck} message 
to the reader. 
Therefore, 
$|\srvSet|^{2} + 2|\srvSet|$
messages are exchanged in any read operation.
% in both algorithms \osam{} (SWMR) and algorithm \omam (MWMR). 

SWMR and MWMR read operation message complexity in algorithms \osamex{} and \omamex{}:
%\paragraph{} \emph{Extended Read operation message complexity (SWMR and MWMR).} 
%From the communication complexity analysis we know that in the \emph{worst-case} scenario all 
Read operations in the worst case take \emph{3} communication exchanges. 
The first exchange occurs when a reader sends a \emph{readRequest} message 
to all servers in $\srvSet$. 
The second exchange occurs when  servers in $\srvSet$ send \emph{readRelay} 
messages to all servers in $\srvSet$ and to the reader. 
The final exchange occurs when servers in $\srvSet$ send 
a \emph{readAck} message to the reader. 
%
Summing together $|\srvSet| + (|\srvSet|^{2} + |\srvSet|)+ |\srvSet|$ gives
$|\srvSet|^{2} + 3|\srvSet|$ 
messages that are exchanged in the worst case during any read operation.
% in both algorithms \osamex{} (SWMR) and algorithm \omamex (MWMR). 


